High spin states of $^{204}$At: isomeric states and shears band structure

High-spin states of neutron deficient Trans-Lead nucleus $^{204}$At were populated up to $\sim 8\,{\rm MeV}$ excitation through the $^{12}$C + $^{197}$Au fusion evaporation reaction. Decay of the associated levels through prompt and delayed $\gamma$-ray emissions were studied to evaluate the underlying nuclear structure. The level scheme, which was partly known, was extended further. An isomeric $16^+$ level with observed lifetime $\tau=52 \pm 5\, {\rm ns}$, was established from our measurements. Attempts were made to interpret the excited states based on multi quasiparticle and hole structures involving $2f_{5/2}$, $1h_{9/2}$, and $1i_{13/2}$ shell model states, along with moderate core excitation. Magnetic dipole band structure over the spin parity range:~$16^+ - 23^+$ was confirmed and evaluated in more detail, including the missing cross-over $E2$ transitions. Band-crossing along the shears band was observed and compared with the evidence of similar phenomena in the neighbouring neutron deficient $^{202}$Bi, $^{205}$Rn isotones and the $^{203}$At isotope. Based on comparison of the measured $B(M1)/B(E2)$ values for transitions along the band with the semiclassical model based estimates, the shears band of $^{204}$At was established along with the level scheme.

==> main.tex <==
\input{204AtEPJv5.tex}

